$\mathsf{QuITO}$ $\textsf{v.2}$: Trajectory Optimization with Uniform Error Guarantees under Path Constraints

This article introduces a new transcription, change point localization, and mesh refinement scheme for direct optimization-based solutions and for uniform approximation of optimal control trajectories associated with a class of nonlinear constrained optimal control problems (OCPs). The base transcription algorithm for which we establish the refinement algorithm is a direct multiple shooting technique -- $\mathsf{QuITO}$ $\textsf{v.2}$ (Quasi-Interpolation based Trajectory Optimization). The mesh refinement technique consists of two steps -- localization of certain irregular regions in an optimal control trajectory via wavelets, followed by a targeted $h$-refinement approach around such regions of irregularity. Theoretical approximation guarantees on uniform grids are presented for optimal controls with certain regularity properties, along with guarantees of localization of change points by wavelet transform. Numerical illustrations are provided for control profiles involving discontinuities to show the effectiveness of the localization and refinement strategy. We also announce, and make freely available, a new software package based on $\mathsf{QuITO}$ $\textsf{v.2}$ along with all its functionalities for completeness. The package is available at: https://github.com/chatterjee-d/QuITOv2.git.

==> NumExp6.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Path constrained OCP %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \subsection{Path Constrained OCP}\label{num:pathconstrainedOCP}
%  Consider the optimal control problem \cite{ref:software_MISER_3_update} with a time-varying path constraint:
% \begin{equation}
% \label{eq:pathC_OCP_con}
% \begin{aligned}
% & \minimize_{\cont(\cdot)}	&&  \int_{0}^{1} \left(\st_1(t)^2 + \st_2(t)^2 +  0.005\cont(t)^2\right)\, \dd t \\
% &  \sbjto		&&  \begin{cases}
% \dot{\st}_1(t)=\st_2(t),\\
% \dot{\st}_2(t)= - \st_2(t) + \cont(t),\\
% \st(0)^{\top} =  (0 \,\, -1)^{\top} \\
% |\st_1(t)| \le 10,\, \,|\st_2(t)| \le 10, \, \, |u(t)| \le 1 \\
% 8(t-0.5)^2 - 0.5 - \st_2(t) \ge 0.
% \end{cases}
% \end{aligned}
% \end{equation}
% The optimal control trajectory features an initial sharp decrease followed by two sharp kinks at \(\{0.29,0.7\}.\). We aim to accurately capture such high-frequency behaviour, particularly these kinks through targeted mesh refinement. We start with a uniform grid with \(\Ninit=100\). We can see that the detection algorithm accurately localizes the initial sharp decrease and kinks with wavelet modulus maxima located at  \(\tau = \aset[]{0.031,0.275, 0.708}\) in Figure \eqref{fig:PCwaveletandmesh}. Corresponding mesh refinement history, cost over iterations, and the solution trajectories are plotted for reference. In Figure \eqref{fig:PCcontrol}, we compare the mesh refinement solution with \(\quito\) solution on a denser uniform grid (\(\Ninit=200\)) and the ICLOCS2 direct collocation solution with mesh refinement (\(N=100\) steps). The corresponding optimization statistics are collected in Table \eqref{vdo:PC-cpu-time}. It is visible that with mesh refinement, sharp behaviour is accurately captured and the solution trajectory converges to the ICLOCS2 solution. In fact, without mesh refinement, we see that a fine discretization approach, i.e., even with a 100\% denser uniform grid (\(N=200\) steps), the baseline-\(\quito\) solution obtains solution trajectory with a higher cost, while also taking more time for computation. This highlights the need and effectiveness of our detection and mesh refinement algorithm.

% \begin{figure}[htpb]
% \includegraphics[width=0.49\textwidth]{results/PC_detection.eps}
% % \hspace{\fill}
% \includegraphics[width=0.49\textwidth]{results/PC_mesh.eps}
% \caption{Wavelet coefficients for a set of scales of order \(10^{-3}\) (left) and mesh history during refinement (right) for Example \ref{num:pathconstrainedOCP}.}\label{fig:PCwaveletandmesh}
% \end{figure}

% \begin{figure}[htpb]
% \includegraphics[width=0.49\textwidth]{results/PC_cost.eps}
% % \hspace{\fill}
% \includegraphics[width=0.49\textwidth]{results/PC_states.eps}
% \caption{Cost variation on each refinement iteration (left) and state trajectories after refinement(right) for Example \ref{num:pathconstrainedOCP}.Underlying grid is shown in green marker}\label{fig:PCcostandstate}
% \end{figure}

% \begin{figure}[htpb]
% \includegraphics[width=12cm,height=8cm]{results/PC_control_smoothedbr.eps}
% \caption{ Control trajectories obtained using refinement for Example \ref{num:pathconstrainedOCP}.}\label{fig:PCcontrol}
% \end{figure}



% \begin{table}[h!]
% \caption{A comparison of optimization statistics for Example \ref{num:pathconstrainedOCP}.}
% \begin{tblr}{l c c c}
% 	\hline[2pt]
% 		\SetRow{azure9}\SetCell[c=4]{c} CPU time, Grid size, cost comparison
% & 3-2
% & 3-3
% & 3-4
% \\
% \hline[1pt]
% Method & \(\Ninit\) &  Minimized cost & CPU time \\ 
% \hline
% \(\quito\) with mesh refinement &  100 &  0.1709   & 182.0859 sec\\
%  \hline
%  \(\quito\) without mesh refinement & 200  & 0.1722 &  351.47 sec\\
%  \hline
% ICLOCS2 with mesh refinement & 100  &  0.1699  & 4 sec \\
% \hline[2pt]
%  % ICLOCS2 without mesh-refinement & 200  &  0.1698  & 0.5964 sec \\
%  % \hline[2pt]
% \end{tblr}
% \centering
% \label{vdo:PC-cpu-time}
% \end{table}

==> NumExp9.tex <==
\subsection{The robot arm rehabilitation problem}



==> dtb.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Facts centered around the double tangent bundle}
\label{s:dtb}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

With the tangent bundle \(\tanbundle\manifold\) of \(\manifold\) endowed with its natural smooth structure, it is possible to consider the double tangent bundle \(\dtanbundle\manifold\) of \(\manifold\). One naturally gets the following commutative diagram (that \cite[p.\ 48]{ref:AbrMar-78} calls the ``dual tangent rhombic'',) illustrating two natural vector bundle structures \(\dtanbundle\manifold\xrightarrow{\vproj{\tanbundle\manifold}} \tanbundle\manifold\) and \(\dtanbundle\manifold\xrightarrow{\tangent\vproj{\manifold}} \tanbundle\manifold\) on \(\dtanbundle\manifold\):
\[
	\begin{tikzcd}[column sep=normal, row sep=normal]
		& \dtanbundle\manifold \arrow[dl, "\vproj{\tanbundle\manifold}"'] \arrow[dr, "\tangent\vproj{\manifold}"] & \\
		\tanbundle\manifold \arrow[dr, "\vproj{\manifold}"'] & & \tanbundle\manifold \arrow[dl, "\vproj{\manifold}"]\\
		& \manifold & 
	\end{tikzcd}
\]
The composite of the left-hand vertical chain \(\dtanbundle\manifold \xrightarrow[]{\vproj{\tanbundle\manifold}} \tanbundle\manifold \xrightarrow[]{\vproj{\manifold}} \manifold\) and the right-hand vertical chain \(\dtanbundle\manifold \xrightarrow[]{\tangent \vproj{\manifold}} \tanbundle\manifold \xrightarrow[]{\vproj{\manifold}} \manifold\) yield two bundles that we shall consider next. We refer to \cite[\S8]{ref:Mic-08} for some of the details.

%%==============================================================================
\subsection{The bundle \(\dtanbundle{\manifold}\xrightarrow[]{\vproj{\tanbundle\manifold}} \tanbundle\manifold \xrightarrow[]{\vproj\manifold} \manifold\)}
%%==============================================================================

With \(\atlas{A} = \aset[\big]{(U_\alpha, \varphi_\alpha)}\) the smoothness on \(\manifold\), the tangent bundle \(\tanbundle\manifold\) is equipped with the natural smoothness 
\[
	\tangent\atlas{A} \Let \aset[\big]{(\tanbundle U, \tangent\varphi)\suchthat (U, \varphi)\in\atlas{A}},
\]
where
\[
	\tanbundle U = U\times\R[d] \ni (x, v)\mapsto (\tangent\varphi)(x, v) = \bigl(\varphi(x), (\tangent_x\varphi)(v)\bigr)\in \varphi(U)\times\R[d] = \tanbundle{\bigl(\varphi(U)\bigr)}.
\]
The double tangent bundle \(\dtanbundle\manifold\) is thereafter equipped with the vector bundle atlas 
\[
	\dtangent\atlas{A} \Let \aset[\big]{\bigl(\dtanbundle U, \dtangent\varphi\bigr)\suchthat (U, \varphi)\in\atlas{A}},
\]
where
\begin{multline*}
	\dtanbundle U = (U\times \R[d])\times(\R[d]\times\R[d]) \ni (x, v, v_1, v_2)\mapsto (\dtangent\varphi)(x, v, v_1, v_2)\\
	= \Bigl(\bigl(\varphi(x), (\tangent_x\varphi)(v)\bigr), \Bigl((\tangent_x\varphi)(v_1), \bigl(\tangent_{x}\bigl(\tangent\varphi(\cdot, v)\bigr)\bigr)(v_1) + (\tangent_x\varphi)(v_2)\Bigr) \Bigr)\\
	\in (\varphi(U)\times\R[d])\times(\R[d]\times\R[d]) = \dtanbundle{\bigl(\varphi(U)\bigr)}.
\end{multline*}
In particular, if \(U\) and \(\wt U\) are (subsets of \(\R[d]\) and) overlapping local coordinates of \(\manifold\) with \(\varphi:U\lra\wt U\) the smooth diffeomorphism (local coordinate change), then the corresponding vector bundle transition map is
\begin{multline*}
	\dtanbundle U \ni (x, v, v_1, v_2)\mapsto \dtangent \varphi(x, v, v_1, v_2)\\
	= \Bigl( \varphi(x), (\partial_x \varphi)(x)\cdot v, (\partial_x \varphi)(x)\cdot v_1, \bigl(\partial^2_{xx} \varphi\bigr)(x)\cdot v_1\cdot v + (\partial_x \varphi)(x)\cdot v_2\Bigr)\in\dtanbundle{\wt U},
\end{multline*}
which clearly shows the linear structure of the map \((v_1, v_2)\mapsto \dtangent\varphi(x, v, v_1, v_2)\) (since \((x, v)\)) is the base point, demonstrating that the bundle \(\dtanbundle\manifold\xrightarrow[]{\vproj{\tanbundle\manifold}} \tanbundle\manifold\) is indeed a vector bundle.

We observe that the bundle \(\dtanbundle\manifold \xrightarrow[]{\vproj{\manifold}\circ\vproj{\tanbundle\manifold}} \manifold\) is \emph{not} a vector bundle. Indeed, for any local coordinates \(U\) and \(\wt U\) (subsets of \(\R[d]\)) with \(\varphi:U\lra\wt U\) a smooth diffeomorphism, the transformation rule
\begin{multline*}
	\dtanbundle U\ni (x, v, v_1, v_2)\mapsto \dtangent\varphi(x, v, v_1, v_2)\\
	= \Bigl(\varphi(x), (\partial_x\varphi)(x)\cdot v, (\partial_x\varphi)(x)\cdot v_1, \bigl(\partial^2_{xx}\varphi\bigr)(x)\cdot v_1\cdot v + (\partial_x\varphi)(x)\cdot v_2\Bigr)\in\dtanbundle{\wt U}
\end{multline*}
contains the \emph{bilinear} map \(\bigl(\partial^2_{xx}\varphi\bigr)(x)\), and the map \((v, v_1, v_2)\mapsto \dtangent\varphi(x, v, v_1, v_2)\) is not linear as a consequence.

%%==============================================================================
\subsection{The bundle \(\dtanbundle\manifold\xrightarrow[]{\tangent \vproj{\manifold}} \tanbundle\manifold \xrightarrow[]{\vproj\manifold} \manifold\)}
%%==============================================================================

With \(\atlas{A} = \aset[\big]{(U_\alpha, \varphi_\alpha)}\) the smoothness on \(\manifold\), the tangent bundle \(\tanbundle\manifold\) is equipped with the natural smoothness 
\[
	\tangent\atlas{A} \Let \aset[\big]{(\tanbundle U, \tangent\varphi)\suchthat (U, \varphi)\in\atlas{A}},
\]
where
\[
	\tanbundle U = U\times\R[d] \ni (x, v)\mapsto (\tangent\varphi)(x, v) = \bigl(\varphi(x), (\tangent_x\varphi)(v)\bigr)\in \varphi(U)\times\R[d] = \tanbundle{\bigl(\varphi(U)\bigr)}.
\]
As usual, the double tangent bundle \(\dtanbundle\manifold\) is thereafter equipped with the vector bundle atlas 
\[
	\dtangent\atlas{A} \Let \aset[\big]{\bigl(\dtanbundle U, \dtangent\varphi\bigr)\suchthat (U, \varphi)\in\atlas{A}},
\]
where
\begin{multline*}
	\dtanbundle U = (U\times \R[d])\times(\R[d]\times\R[d]) \ni (x, v, v_1, v_2)\mapsto (\dtangent\varphi)(x, v, v_1, v_2)\\
	= \Bigl(\bigl(\varphi(x), (\tangent_x\varphi)(v)\bigr), \Bigl((\tangent_x\varphi)(v_1), \bigl(\tangent_{x}\bigl(\tangent\varphi(\cdot, v)\bigr)\bigr)(v_1) + (\tangent_x\varphi)(v_2)\Bigr) \Bigr)\\
	\in (\varphi(U)\times\R[d])\times(\R[d]\times\R[d]) = \dtanbundle{\bigl(\varphi(U)\bigr)}.
\end{multline*}
In particular, if \(U\) and \(\wt U\) are (subsets of \(\R[d]\) and) overlapping local coordinates of \(\manifold\) with \(\varphi:U\lra\wt U\) the smooth diffeomorphism (local coordinate change), then the corresponding base point is
\[
	\dtanbundle U\ni (x, v, v_1, v_2)\mapsto \tangent\vproj{\manifold}(x, v, v_1, v_2) = (x, v_1),
\]
and the vector bundle transition map is
\begin{multline*}
	\dtanbundle U \ni (x, v, v_1, v_2)\mapsto \dtangent \varphi(x, v, v_1, v_2)\\
	= \Bigl( \varphi(x), (\partial_x \varphi)(x)\cdot v, (\partial_x \varphi)(x)\cdot v_1, \bigl(\partial^2_{xx} \varphi\bigr)(x)\cdot v_1\cdot v + (\partial_x \varphi)(x)\cdot v_2\Bigr)\in\dtanbundle{\wt U},
\end{multline*}
which clearly shows that the map \((v, v_2)\mapsto \dtangent\varphi(x, v, v_1, v_2)\) is linear since the base point is \((x, v_1)\). This calculation also shows that the bundle \(\dtanbundle\manifold\xrightarrow[]{\vproj{\manifold}\circ\tangent\vproj{\manifold}} \manifold\) is \emph{not} a vector bundle because the map \((v, v_1, v_2)\mapsto \dtangent\varphi(x, v, v_1, v_2)\) contains the \emph{bilinear} map \(\bigl(\partial^2_{xx}\varphi\bigr)(x)\) at the base point \(x\).

%%==============================================================================
\subsection{The canonical involution}
%%==============================================================================

Associated with the double tangent bundle \(\dtanbundle \manifold\) there is the smooth map \(\canoflip:\dtanbundle\manifold\lra\dtanbundle\manifold\), called the \embf{canonical flip} or the \embf{canonical involution}, defined locally as follows: If \(U\subset\R[d]\) is open, then
\begin{equation}
	\label{e:canoflip}
	\dtanbundle U\ni (x, v, v_1, v_2)\mapsto \canoflip(x, v, v_1, v_2) \Let (x, v_1, v, v_2)\in \dtanbundle U.
\end{equation}
We quickly verify the transformation rule for \(\canoflip\): If \(U\ni x\mapsto \varphi(x)\in \wt U\) is a smooth diffeomorphism, then \(\tanbundle U\ni (x, v)\mapsto (\tangent\varphi)(x, v) = \bigl(\varphi(x), (\totder{x}\varphi)(x)\cdot v\bigr)\in \tanbundle{\wt U}\) is the tangent map and 
\begin{multline*}
	\dtanbundle U\ni (x, v, v_1, v_2)\mapsto (\dtangent\varphi)(x, v, v_1, v_2)\\
	= \Bigl(\varphi(x), (\totder{x}\varphi)(x)\cdot v, (\totder{x}\varphi)(x)\cdot v_1, \bigl(\totder{xx}^2\varphi\bigr)(x)\cdot v_1\cdot v + (\totder{x}\varphi)(x)\cdot v_2\Bigr)\in\dtanbundle{\wt U}
\end{multline*}
is the double tangent map, then from the fact that \(\bigl(\partial^2_{xx}\varphi\bigr)(x)\) is a symmetric map, it follows that
\begin{multline*}
	\canoflip\Bigl(\varphi(x), (\totder{x}\varphi)(x)\cdot v, (\totder{x}\varphi)(x)\cdot v_1, \bigl(\totder{xx}^2\varphi\bigr)(x)\cdot v_1\cdot v + (\totder{x}\varphi)(x)\cdot v_2\Bigr)\\
	= \Bigl(\varphi(x), (\totder{x}\varphi)(x)\cdot v_1, (\totder{x}\varphi)(x)\cdot v, \bigl(\totder{xx}^2\varphi\bigr)(x)\cdot v_1\cdot v + (\totder{x}\varphi)(x)\cdot v_2\Bigr),
\end{multline*}
which shows that the definition of the canonical involution is coordinate-invariant; i.e., \(\dtangent\varphi\circ \canoflip = \canoflip\circ\dtangent\varphi\). Moreover, the following diagrams commute:
\begin{equation}
	\label{e:canoflip2}
	\begin{tikzcd}[column sep=small, row sep=normal]
		\dtanbundle \manifold \arrow[dr, "\vproj{\tanbundle\manifold}"'] \arrow[rr, "\canoflip"] & & \dtanbundle\manifold \arrow[dl, "\tangent\vproj{\manifold}"] \\
		& \tanbundle\manifold &
	\end{tikzcd}
	\quad
	\begin{tikzcd}[column sep=small, row sep=normal]
		\dtanbundle \manifold \arrow[dr, "\tangent\vproj{\manifold}"'] \arrow[rr, "\canoflip"] & & \dtanbundle\manifold \arrow[dl, "\vproj{\tanbundle\manifold}"] \\
		& \tanbundle\manifold &
	\end{tikzcd}
\end{equation}
and, in particular, \(\canoflip\circ\canoflip = \id\) as is evident from the local definition of \(\canoflip\). The canonical involution is, therefore, an isomorphism between the two vector bundles \(\dtanbundle\manifold\xrightarrow[]{\tangent\vproj{\manifold}} \tanbundle\manifold\) and \(\dtanbundle \manifold\xrightarrow[]{\vproj{\tanbundle\manifold}} \tanbundle\manifold\).

The canonical involution \(\canoflip\) is the unique map \(\dtanbundle\manifold\lra\dtanbundle\manifold\) that satisfies the property:\footnote{This calculation is omitted in \cite[\S8]{ref:Mic-08}.}
\begin{equation}
	\label{e:canoflip property}
	\text{for all smooth }c:\R[2]\lra\manifold\text{ we have}\quad \frac{\partial}{\partial t} \frac{\partial}{\partial s} c(t, s) = \canoflip \Bigl( \frac{\partial}{\partial s} \frac{\partial}{\partial t} c(t, s) \Bigr).
\end{equation}
This preceding identity is the analog of Schwarz's identity concerning the commutation of partial derivatives on Euclidean spaces; it is clear from \eqref{e:canoflip property} that a bit more care is needed for Schwarz's identity on smooth manifolds.

Since it suffices to prove \eqref{e:canoflip property} in local coordinates, assume that \(U\subset\R[d]\) is an open set and let \(\R[2]\ni (t, s)\mapsto c(t, s)\in U\) is a smooth map. Then, on the one hand,
\[
	\R[2]\ni (t, s) \mapsto \frac{\partial}{\partial t} c(t, s) = \Bigl( c(t, s), \frac{\partial}{\partial \tau}\Bigr|_{\tau=0} c(t+\tau, s)\Bigr) \in \tanbundle U
\]
and consequently,
\begin{align*}
	& \R[2]\ni (t, s) \mapsto \frac{\partial}{\partial s} \frac{\partial}{\partial t} c(t, s)\\
	& = \Bigl( c(t, s), \frac{\partial}{\partial\tau}\Bigr|_{\tau=0} c(t+\tau, s), \frac{\partial}{\partial \sigma}\Bigr|_{\sigma=0} c(t, s+\sigma), \frac{\partial}{\partial\sigma}\Bigr|_{\sigma=0} \frac{\partial}{\partial\tau}\Bigr|_{\tau=0} c(t+\tau, s+\sigma)\Bigr)\in\dtanbundle U.
\end{align*}
On the other hand,
\[
	\R[2]\ni (t, s) \mapsto \frac{\partial}{\partial s} c(t, s) = \Bigl( c(t, s), \frac{\partial}{\partial\sigma}\Bigr|_{\sigma=0} c(t, s+\sigma)\Bigr) \in \tanbundle U
\]
and consequently,
\begin{align*}
	& \R[2]\ni (t, s) \mapsto \frac{\partial}{\partial t} \frac{\partial}{\partial s} c(t, s)\\
	& = \Bigl( c(t, s), \frac{\partial}{\partial\sigma}\Bigr|_{\sigma=0} c(t, s+\sigma), \frac{\partial}{\partial\tau}\Bigr|_{\tau=0} c(t+\tau, s), \frac{\partial}{\partial\tau}\Bigr|_{\tau=0} \frac{\partial}{\partial\sigma}\Bigr|_{\sigma=0} c(t+\tau, s+\sigma)\Bigr)\in\dtanbundle U.
\end{align*}
The property \eqref{e:canoflip property} is evident from the preceding calculations.


%%==============================================================================
\subsection{The variational vector field}
%%==============================================================================

\begin{prgr}
	If \(\vecfld\) is a smooth vector field on \(\manifold\), then \((\canoflip\circ\tangent\vecfld)\) is a smooth vector field on \(\tanbundle\manifold\). Indeed, it is clear that \((\canoflip\circ\tangent\vecfld):\tanbundle\manifold\lra\dtanbundle\manifold\) is a smooth map, and since
	\begin{align*}
		\vproj{\tanbundle\manifold}\circ(\canoflip\circ\tangent\vecfld) & = (\vproj{\tanbundle\manifold}\circ\canoflip)\circ\tangent\vecfld &&\\
		& = \tangent\vproj{\manifold}\circ\tangent\vecfld && \text{in view of \eqref{e:canoflip2}}\\
		& = \tangent(\vproj{\manifold}\circ\vecfld) && \text{by the chain rule}\\
		& = \tangent\id_{\manifold} && \text{since \(\vproj{\manifold}\circ\vecfld = \id_{\manifold}\)}\\
		& = \id_{\tanbundle\manifold}, &&
	\end{align*}
	it follows that \((\canoflip\circ\tangent\vecfld)\) is a smooth section of \(\dtanbundle\manifold\xrightarrow[]{\vproj{\tanbundle\manifold}} \tanbundle\manifold\) as claimed.
\end{prgr}

The vector field \(\canoflip\circ\tangent\vecfld\) is called the \embf{variational vector field} or the \embf{natural lift} of \(\vecfld\) on \(\tanbundle\manifold\). The flow on \(\tanbundle\manifold\) of \(\canoflip\circ\tangent\vecfld\) is related to the flow on \(\manifold\) of \(\vecfld\) in the following fashion:

\begin{prgr}
	If \(\vecfld\) is a smooth vector field on \(\manifold\) and \((\flow{t})_{t}\) is its flow on \(\manifold\) for \(t\in\R\) sufficiently small, then \((\tangent\flow{t})_{t}\) is the flow of \((\canoflip\circ\tangent\vecfld)\) on \(\tanbundle\manifold\) for as long as \((\flow{t})_{t}\) is defined. We start by observing that since \(\flow{t+s} = \flow{s}\circ\flow{t}\) for all \(t, s\in\R\) sufficiently small and \(\flow{0} = \id_{\manifold}\), we have \(\tangent\flow{s}\circ\tangent\flow{t} = \tangent\flow{s+t}\) and \(\tangent\flow{0} = \id_{\tanbundle\manifold}\). Therefore,
	\[
		\frac{\dd}{\dd t} \tangent\flow{t} = \frac{\dd}{\dd s}\Bigr|_{s=0} \tangent\flow{s}\circ\tangent\flow{t},
	\]
	and defining \(\wt\vecfld \Let \frac{\dd}{\dd s}\big|_{s=0} \tangent\flow{s}\), we arrive at
	\[
		\frac{\dd}{\dd t}\tangent\flow{t} = \wt\vecfld\circ\tangent\flow{t}\quad\text{for all \(t\) sufficiently small},
	\]
	which shows that \(\tangent\flow{(\cdot)}\) is the flow of \(\canoflip\circ\tangent\vecfld\). Finally, from \eqref{e:canoflip property} we get
	\[
		\wt\vecfld = \frac{\dd}{\dd s}\Bigr|_{s=0} \tangent\flow{s} = \canoflip\circ \tangent\biggl( \frac{\dd}{\dd s}\Bigr|_{s=0} \flow{s}\biggr) = \canoflip \circ\tangent\vecfld
	\]
	as asserted. It turns out that the identity \(\wt\vecfld = \canoflip\circ\tangent\vecfld\) is equally easy to derive directly without invoking the analog \eqref{e:canoflip property} of Schwarz's identity. Indeed, if \(U\subset\R[d]\) is an open set, then \(\flow{t}\) is a smooth diffeomorphism on \(U\) for all sufficiently small \(t\in\R[]\). On the one hand, the definition of tangent maps leads to, for \(t\in\R[]\) sufficiently small,
	\begin{align*}
		& U\ni y\mapsto \flow{t}(y)\in \flow{t}(U)\quad\text{and}\\
		& \tanbundle U\ni (y, w) \mapsto \tangent\flow{t}(y, w) = \bigl(\flow{t}(y), \partial_y\flow{t}(y)\cdot w\bigr)\in\tanbundle{\bigl(\flow{t}(U)\bigr)} = \flow{t}(U)\times\R[d];
	\end{align*}
	consequently, for \(\eps > 0\) small enough and with \(\bar\vecfld\) representing the principal part of \(\vecfld\),
	\begin{multline*}
		\loro{-\eps}{\eps}\times\R\ni (t, s) \mapsto \tangent\bigl( \tangent\flow{(\cdot)}(y, w) \bigr) (t, s) = \frac{\partial}{\partial t} \tangent\flow{t}(y, w)\cdot s\\
		= \Bigl( \bigl(\flow{t}(y), \partial_y\flow{t}(y)\cdot w\bigr), \Bigl( \bar\vecfld\bigl(\flow{t}(y)\bigr) \cdot s, \partial_y\bar\vecfld\bigl(\flow{t}(y)\bigr)\cdot s\cdot w\Bigr) \Bigr)\\
		\in\dtanbundle{\bigl(\flow{t}(U)\bigr)} = \flow{t}(U)\times\R[d]\times\R[d]\times\R[d],
	\end{multline*}
	where we employed the standard Schwarz's identity on Euclidean spaces. Since \(\flow{0} = \id_{U}\), evaluating at \(t = 0\) and \(s = 1\) we get
	\[
		\tangent\bigl( \tangent\flow{(\cdot)}(y, w) \bigr) (0, 1) \overset{(\dag)}{=} \bigl( y, w, \bar\vecfld(y), \partial_y\bar\vecfld(y)\cdot w\bigr)\in\dtanbundle U.
	\]
	On the other hand, considering the vector field \(\vecfld\) directly, we have
	\begin{align*}
		& U\ni y\mapsto \vecfld(y) = \bigl(y, \bar\vecfld(y)\bigr)\in\tanbundle U \quad\text{and}\\
		& \tanbundle U\ni (y, w) \mapsto \tangent\vecfld(y, w) = \bigl( \vecfld(y), \partial_y\vecfld(y)\cdot w \bigr) = \Bigl( y, \bar\vecfld(y), w, \partial_y\bar\vecfld(y)\cdot w\Bigr)\in\dtanbundle U,
	\end{align*}
	and it follows at once from \((\dag)\) that \((\canoflip\circ\tangent\vecfld)(y, w) = \tangent\bigl( \tangent\flow{(\cdot)}(y, w) \bigr) (0, 1)\) as asserted.
\end{prgr}

In other words, the local formula of the natural lift \(\canoflip\circ\tangent\vecfld\) of \(\vecfld\) in terms of the local fomula of \(\vecfld\) is
\begin{equation}
	\label{e:variational vecfld local}
	\begin{aligned}
		& U\ni x\mapsto \vecfld(x) = \bigl(x, \bar\vecfld(x)\bigr)\in\tanbundle U\\
		& \tanbundle U\ni (x, v) \mapsto (\canoflip\circ\tangent\vecfld)(x, v) = \Bigl( \bigl( x, \bar\vecfld(x) \bigr), \bigl( \bar\vecfld(x), (\totder{x}\bar\vecfld)(x)\cdot v \bigr) \Bigr) \in\dtanbundle U.
	\end{aligned}
\end{equation}
Recall \cite[Chapter 1]{ref:YanIsh-73} that the \emph{complete lift} \(\xi\complift\) of a smooth vector field \(\xi:\manifold\lra\tanbundle\manifold\) is defined by the equality
\[
	\xi\complift\bigl(\ii(\dd\varphi)\bigr) = \bigl(\xi(\varphi)\bigr)\complift \quad\text{for all smooth functions \(\varphi\)},
\]
where \(\omega\mapsto\ii\omega\) is the natural lift of a \(1\)-form \(\omega\) to the tangent bundle \(\tanbundle\manifold\) on which \(\ii\omega\) is regarded as a smooth function, and the complete lift \(\varphi\complift\) of a smooth function \(\varphi:\manifold\lra\R\) to \(\tanbundle\manifold\) is defined by \(\varphi\complift \Let \varphi\circ\vproj{\manifold}\). In local coordinates, if \(U\subset\R[d]\) is an open set, then
\begin{align*}
	& U\ni x\mapsto \varphi(x)\in\R\quad\text{is a smooth function},\\
	& \tanbundle U\ni (x, v) \mapsto \dd\varphi(x)\cdot v \Let \inprod{\totder{x}\varphi(x)}{v},\\
	& \tanbundle U\ni (x, v) \mapsto \ii(\dd\varphi)(x, v) \Let \dd\varphi(x)\cdot v,\\
	& U\ni x\mapsto \xi(x) \Let \bigl(x, \bar\xi(x)\bigr)\in\tanbundle U\quad\text{is a smooth vector field},
\end{align*}
and if \(\tanbundle U\ni (x, v)\mapsto \xi\complift(x, v) \Let \Bigl(x, v, \bigl(\bar\xi_1(x, v), \bar\xi_2(x, v)\bigr)\Bigr)\in\dtanbundle U\) is the complete lift of \(\xi\) in these local coordinates for smooth maps \(\bar\xi_1, \bar\xi_2:\tanbundle U\lra\R[d]\) that are to be determined, then then the defining equality forces
\begin{align*}
	\xi\complift\bigl(\ii(\dd\varphi)\bigr)(x, v) & = \totder{(x, v)}\bigl(\ii(\dd\varphi)\bigr)(x, v)\cdot\bigl(\bar\xi_1(x, v), \bar\xi_2(x, v)\bigr)\\
	& = (\totder{xx}^2\varphi)(x)\cdot \bar\xi_1(x, v)\cdot v + (\totder{x}\varphi)(x)\cdot\bar\xi_2(x, v)
	\intertext{to be equal to, for all smooth \(\varphi\),}
	\bigl(\xi(\varphi)\bigr)\complift(x, v) & = \bigl(\totder{(x, v)}\LieD{\xi}\varphi\bigr)(x, v)\cdot (x, v)\\
	& = \bigl( \totder{(x, v)} (\totder{x}\varphi)(x)\cdot \bar\xi(x) \bigr)(x, v)\\
	& = (\totder{xx}^2\varphi)(x)\cdot v\cdot\bar\xi(x) + (\totder{x}\varphi)(x)\cdot(\totder{x}\bar\xi)(x)\cdot v.
\end{align*}
It follows at once from elementary calculations and the fact that \((\totder{xx}^2\varphi)(x)\) is a symmetric bilinear map that \(\bar\xi_1(x, v) = \bar\xi(x)\) and \(\bar\xi_2(x, v) = (\totder{x}\varphi)(x)\cdot v\). An inspection of the local expression \eqref{e:variational vecfld local} of the variational vector field \(\canoflip\circ\tangent\vecfld\) is sufficient to conclude that \(\vecfld\complift = \canoflip\circ\tangent\vecfld\); we shall write \(\vecfld\complift\) for the variational vector field henceforth.

%%==============================================================================
\subsection{Splitting of \(\dtanbundle\manifold\)}
%%==============================================================================

We quickly review the splitting of the double tangent bundle due to Dombrowski \cite[Chapter X]{ref:Lan-99}. Let the smooth manifold \(\manifold\) be equipped with a covariant derivative, and \(\R\)-bilinear map 
\[
	\smoothvf{\manifold}\times\smoothvf{\manifold}\ni (\xi, \eta) \mapsto \covder{}{}(\xi, \eta) \Let \covder{\xi}{\eta} \in\smoothvf{\manifold}
\]
such that
\begin{itemize}[label=\(\circ\)]
	\item if \(\varphi:\manifold\lra\R\) is smooth, then we set \(\covder{\xi}{\varphi} \Let \LieD{\xi}{\varphi}\) by definition,
\end{itemize}
and stipulate that the following three properties hold:
\begin{itemize}[label=\(\circ\)]
	\item \(\covder{\varphi\xi}{\eta} = \varphi \covder{\xi}{\eta}\), i.e., \(\covder{(\cdot)}{\eta}\) is linear with respect to scaling by smooth functions,
	\item \(\covder{\xi}{(\varphi\eta)} = (\covder{\xi}\varphi)\eta + \varphi \covder{\xi}{\eta}\), i.e., \(\covder{\xi}{(\cdot)}\) is a derivation, and
	\item \(\covder{\xi}{\eta} - \covder{\eta}{\xi} = \LieBracket{\xi}{\eta}\) (known as the `torsion-free' property).
\end{itemize}
It is well known \cite[Theorem 2.4, Chapter VIII]{ref:Lan-99} that corresponding to the covariant derivative \(\covder{}{}\) there exists a unique smooth spray \(\spray:\tanbundle\manifold\lra\dtanbundle\manifold\). We shall represent the symmetric bilinear map associated with this spray in a local chart \(U\subset\R[d]\) as \(\blmap_U\). The relationship between the covariant derivative \(\covder{}{}\) and \(\blmap\) is given by
\[
	(\covder{\xi}{\eta})_U(x) = (\totder{x}\eta_U)(x) \cdot \xi_U(x) - \blmap_U\bigl(x; \xi_U(x), \eta_U(x)\bigr)\quad \text{for all }\xi, \eta\in\smoothvf{\manifold},
\]
where \(\xi_U\) and \(\eta_U\) are local representatives of \(\xi\) and \(\eta\) on \(U\). We recall here the Dombrowski splitting Theorem:
\begin{theorem}[{\cite[Theorem 4.5, Chapter X]{ref:Lan-99}}]
	Let \(\manifold\) be a \(d\)-dimensional smooth manifold equipped with a smooth spray \(\spray\), and let \(\tanbundle\manifold\xrightarrow[]{\vproj{\manifold}} \manifold\) and \(\dtanbundle\manifold\xrightarrow[]{\vproj{\tanbundle\manifold}} \tanbundle\manifold\) be its tangent and double tangent bundles, respectively. Let the symmetric bilinear map associated with the spray \(\spray\) in a local chart \(U\subset\R[d]\) be denoted by \(\blmap_U\). Then there exists a unique vector bundle morphism \(\vertmap:\dtanbundle\manifold\lra\tanbundle\manifold\) given in the chart \(U\) by
	\[
		\R[d]\times\R[d]\ni (v_1, v_2) \mapsto \vertmap(x, v, v_1, v_2) \Let v_2 - \blmap_U(x; v, v_1)\in\R[d] \quad\text{for all }(x, v)\in\tanbundle U.
	\]
	Moreover,
	\begin{equation}
		\label{e:splitting}
		\bigl(\vproj{\tanbundle\manifold}, \tangent\vproj{\manifold}, \vertmap\bigr):\dtanbundle\manifold\lra \tanbundle\manifold\directsum\tanbundle\manifold\directsum\tanbundle\manifold
	\end{equation}
	is an isomorphism of fiber bundles over \(\manifold\).
\end{theorem}

The second and third factors in the splitting \eqref{e:splitting} are the \embf{horizontal} and \embf{vertical} bundles, respectively.


